Learning in Gated Neural Networks

Gating is a key feature in modern neural networks including LSTMs, GRUs and sparsely-gated deep neural networks. The backbone of such gated networks is a mixture-of-experts layer, where several experts make regression decisions and gating controls how to weigh the decisions in an input-dependent manner. Despite having such a prominent role in both modern and classical machine learning, very little is understood about parameter recovery of mixture-of-experts since gradient descent and EM algorithms are known to be stuck in local optima in such models. In this paper, we perform a careful analysis of the optimization landscape and show that with appropriately designed loss functions, gradient descent can indeed learn the parameters accurately. A key idea underpinning our results is the design of two {\em distinct} loss functions, one for recovering the expert parameters and another for recovering the gating parameters. We demonstrate the first sample complexity results for parameter recovery in this model for any algorithm and demonstrate significant performance gains over standard loss functions in numerical experiments.

==> Zipping for arXiv/discussion.tex <==
% !TEX root = gated_moe.tex
\section{Discussion}
\label{sec:disc}

In this paper we established the first mathematical connection between two popular gated neural networks: GRU and MoE. Inspired by this connection and the success of SGD based algorithms in finding global minima in a variety of non-convex problems in deep learning, we provided the first gradient descent based approach for learning the parameters in a MoE. While the canoncial MoE does not involve any time series, extension of our methods for the recurrent setting is an important future direction. Similarly, extensions to deep MoE comprised of multiple gated as well as non-gated layers is also a fruitful direction of further research. We believe that the theme of using different loss functions for distinct parameters in NN models can potentially enlighten some new theoretical insights as well as practical methodologies for complex neural models.

==> Zipping for arXiv/experiments.tex <==
% !TEX root = gated_moe.tex
\section{Experiments}
\label{sec:experiments}


In this section, we empirically validate the fact that running SGD on our novel loss functions $L_4$ and $L_\mathrm{\log}$ achieves superior performance compared to the existing approaches. Moreover, we empirically show that our algorithms are robust to the technical assumptions made in \prettyref{thm:landscape} and that they achieve equally good results even when the assumptions are relaxed.

{\bf Data generation.} For our experiments, we choose $d=10$, $k \in \{2,3\}$, $\ba_i^\ast=\be_i$ for $i \in [k]$ and $\bw_i^\ast=\be_{k+i}$ for $i \in [k-1]$, and $g=\Id$. We generate the data $\{(\bx_i,y_i)_{i=1}^n \}$ according to \prettyref{eq:kmoe} and using these ground-truth parameters. We chose $\sigma=0.05$ for all of our experiments.

{\bf Error metric.} If $\bA \in \reals^{k \times d}$ denotes the matrix of regressors where each row is of norm $1$, we use the error metric $\calE_{\mathrm{reg}}$ to gauge the closeness of $\bA$ to the ground-truth $\bA^\ast$:
\begin{align*}
\calE_{\mathrm{reg}} \define 1- \max_{\pi \in S_k} \min_{i \in [k]} |\inner{\ba_i}{\ba^\ast_{\pi(i)}}|,
\end{align*}
where $S_k$ denotes the set of all permutations on $[k]$. Note that $\calE_{\mathrm{reg}} \leq \varepsilon$ if and only if the learnt regressors have a minimum correlation of $1-\varepsilon$ with the ground-truth parameters, upto a permutation. The error metric $\calE_{\mathrm{gating}}$ is defined similarly.

{\bf Results.} In \prettyref{fig:regresslearn}, we choose $k=3$ and compare the performance of our algorithm against existing approaches. In particular, we consider three methods: 1) EM algorithm, 2) SGD on the the classical $\ell_2$-loss from \prettyref{eq:l2_loss}, and 3) SGD on our losses $L_4$ and $L_{\mathrm{log}}$. For all the methods, we ran $5$ independent trials and plotted the mean error. \prettyref{fig:all_regressor_error} highlights the fact that minimizing our loss function $L_4$ by SGD recovers the ground-truth regressors, whereas SGD on $\ell_2$-loss as well as EM get stuck in local optima. For learning the gating parameters $W$ using our approach, we first fix the regressors $A$ at the values learnt using $L_4$, \ie $A=\hat{A}$, where $\hat{A}$ is the converged solution for $L_4$. For $\ell_2$ and the EM algorithm, the gating parameters $W$ are learnt jointly with regressors $A$. \prettyref{fig:all_classifier_error} illustrates the phenomenon that our loss $L_{\mathrm{log}}$ for learning the gating parameters performs considerably better than the standard approaches, as indicated in significant gaps between the respective error values. Finally, in \prettyref{fig:our_loss_multiple_runs} we plot the regressor error for $L_4$ over $5$ random initializations. We can see that we recover the ground truth parameters in all the trials, thus empirically corroborating our technical results in \prettyref{sec:optim_landscape}.

%We can also see that SGD is able to escape the saddle points on $L_4$ during the training as highlighted by a plateau around $200$ epochs. We ran the SGD algorithm on both these loss functions with five different runs and plotted the mean error for both.
%%We can see that in all the five runs, SGD on our loss function converges to the ground truth parameters within just a few hundred iterations.
%For learning the gating parameters $W$, we ran SGD on $L_{\mathrm{\log}}$, while fixing the regressors $\bA$ at three different values: $A=\hat{A}$ learned by $L_4$, $A=\hat{A} $ learned by $\ell_2$, and $\bA=\bA^\ast$. From \prettyref{fig:regresslearn} we see that SGD on $L_{\mathrm{log}}$ recovers the true parameters and operates very close to the ground-truth. 




%\begin{figure}
%\includegraphics[width=0.5\textwidth]{k2_d10_batch1024_sample16384_classifier.png}
%\hfill
%\includegraphics[width=0.5\textwidth]{5runs_logloss.png}
%\caption{Learning gating parameters using $L_{\mathrm{\log}}$. Left: Comparison of $\ell_2$ and $L_4$ with ground truth. Right: $5$-different runs of SGD on $L_{\mathrm{\log}}$ using the regressors $\bA$ from $L_4$. }
%\label{fig:classlearn}
%\end{figure}

\subsection{Robustness to technical assumptions}
In this section, we verify numerically the fact that our algorithms work equally well in the absence of technical assumptions made in \prettyref{sec:optim_landscape}.

\textbf{Relaxing orthogonality in \prettyref{thm:landscape}.} A key assumption in proving \prettyref{thm:landscape}, adapted from \cite{makkuva2018breaking}, is that the set of regressors $\{a_i^\ast\}$ and set of gating parameters $\{w_i^\ast\}$ are orthogonal to each other. While this assumption is needed for the technical proofs, we now empirically verify that our conclusions still hold when we relax this. For this experiment, we choose $k=2$ and let $(a_1^\ast, a_2^\ast)=(e_1, e_2)$. For the gating parameter $w^\ast \define w_1^\ast$, we randomly generate it from uniform distribution on the $d$-dimensional unit sphere. In \prettyref{fig:1a} and \prettyref{fig:1b}, we plotted the individual parameter estimation error for $5$ different runs for both of our losses $L_4$ and $L_{\mathrm{log}}$ for learning the regressors and the gating parameter respectively. We can see that our algorithms are still able to learn the true parameters even when the orthogonality assumption is relaxed. 

\textbf{Relaxing Gaussianity of the input.} To demonstrate the robustness of our approach to the assumption that the input $x$ is standard Gaussian, \ie $x \sim \calN(0,I_d)$, we generated $x$ according to a mixture of two symmetric Gaussians each with identity covariances, \ie $x \sim p \calN(\mu, I_d)+(1-p) \calN(-\mu,I_d)$, where  $p \in [0,1]$ is the mixing probability and $\mu \in \reals^d$ is a fixed but randomly chosen vector. For various mixing proportions $p \in \{0.1, 0.2, 0.3, 0.4, 0.5\}$, we ran SGD on our loss $L_4$ to learn the regressors.  \prettyref{fig:1c} highlights that we learn these ground truth parameters in all the settings. 

Finally we note that in all our experiments, the loss $L_4$ seems to require a  larger batch size ($1024$) for its gradient estimation while running SGD. However, with smaller batch sizes such as $128$ we are still able to achieve similar performance but with more variance. (see \prettyref{app:additionalexp}).



%\begin{figure*}
%\includegraphics[width=\textwidth]{non_orth_regress.png}
%\includegraphics[width=\textwidth]{non_orth_class.png}
%
%\caption{Top: Parameter error for regressors using $L_4(\cdot)$. Bottom: Parameter error for gating parameters using $L_{\mathrm{\log}}$}
%\label{fig:non_orthogonal}
%\end{figure*} 

%We also found that similar conclusions hold when we directly compare the performance of $L_{\mathrm{\log}}$ and that of $\ell_2$ for learning $W$.
%Finally we note that the loss $L_4$ seems to require larger batch size ($1024$) for its gradient estimation. However, with smaller batch sizes such as $128$ we are still able to achieve similar performance but with more variance. (see \prettyref{app:additionalexp}).

%in addition to the comparison of our loss vs $\ell_2$, we also compared them against that of the ground-truth. First, using the regressors learnt by $\ell_2$-loss, $L_{4}$ and the ground truth $\bA^\ast$, we ran SGD on $L_{\mathrm{\log}}$ in these three different settings.
%Similarly, we verify that gradient descent on the empirical log-loss yields the ground-truth gating parameters; however, SGD on $\ell_2$-loss is prone to spurious minima. 


==> Zipping for arXiv/gru_as_hMoE.tex <==
% !TEX root = gated_moe.tex
\section{GRU as a hierarchical MoE}
\label{sec:connection}
In this section, we show that the recurrent update equations for GRU can be obtained from that of MoE, described in \prettyref{eq:kmoe}. In particular, we show that GRU can be viewed as a hierarchical MoE with depth-2. To see this, we restrict to the setting of a $2$-MoE, \ie let $k=2$ and $(a_1^\ast, a_2^\ast)= (a_1, a_2)$, and $(w_1^\ast,w_2^\ast)=(w,0)$ in \prettyref{eq:kmoe}. Then we obtain that
\begin{align}
y = (1-z) ~ g(a_1^\top x) + z ~ g(a_2^\top x) + \xi, 
\label{eq:k2moe}
\end{align}
where $z \in \{0,1\} $ and $\prob{z=0|x} = \sigma(w^\top x)$. Since $\xi$ is a zero mean random variable independent of $x$, taking conditional expectation on both sides of \prettyref{eq:k2moe} yields that
\begin{align*}
y(x) & \define \Expect[y|x] \\
&= \sigma(w^\top x)g(a_1^\top x)+(1-\sigma(w^\top x)) g(a_2^\top x) \in \reals.
\end{align*}
Now letting the output $\by(x) \in \reals^m$ to be a vector and allowing for different gating parameters $\{w_i\}$ and regressors $\{(a_{1i},a_{2i})\}$ along each dimension $i =1,\ldots, m$, we obtain
\begin{align}
y(x) = (1-z(x)) \odot g(A_1 x) + z(x) \odot g(A_2 x),
\label{eq:vector_moe}
\end{align}
where $z(x)=(z_1(x),\ldots,z_m(x))^\top$ with $z_i(x)=\sigma(\bw_i^\top \bx)$, and $A_1,A_2 \in \reals^{m\times d}$ denote the matrix of regressors corresponding to first and second experts respectively. 

We now show that \prettyref{eq:vector_moe} is the basic equation behind the updates in GRU. Recall that in a GRU, given a time series $\{(x_t, y_t)\}_{t=1}^T$ of sequence length $T$, the goal is to produce a sequence of hidden states $\{h_t\}$ such that the output time series $\hat{y}_t = f(C h_t)$ is close to $\{y_t\}$ in some well-defined loss metric, where $f$ denotes the non-linear activation of the last layer. The equations governing the transition dynamics between $\{x_t \}$ and $\{h_t\}$ at any time $t \in [T]$ are given by \citep{gru}:
\begin{align*}
h_t = (1-z_t) \odot h_{t-1} +z_t \odot \tilde{h}_t,\\
\tilde{h}_t = g(U_h x_t + W_h (r_t \odot h_{t-1})),
\end{align*}
where $z_t$ and $r_t$ denote the update and reset gates, which are given by
\begin{align*}
 z_t &=\sigma(U_z x_t+W_z h_{t-1}) , \quad  r_t = \sigma(U_r x_t+W_r h_{t-1}),
\end{align*}
where the matrices $U$ and $W$ with appropriate subscripts are parameters to be learnt. While the gating activation function $\sigma$ is modeled as sigmoid for the ease of obtaining gradients while training, their intended purpose was to operate as binary valued gates taking values in $\{0,1\}$. Indeed, in a recent work \cite{li2018towards}, the authors show that binary valued gates enhance robustness with more interpretability and also give better performance compared to their continuous valued counterparts. In view of this, letting $\sigma$ to be the binary threshold function $\mathds{1}\{x \geq 0\}$, we obtain that
\begin{equation}
\begin{aligned}
h_t &= (1-z_t) \odot h_{t-1} + z_t \odot ( (1-r_t)\odot g(U_h x_t) \\
& \hspace{5em} + r_t \odot g(U_h x_t+ W_h h_{t-1})).
\end{aligned}
\label{eq:grumoe}
\end{equation}
Letting $\bx=(\bx_t,\bh_{t-1})$ and $\by(\bx)=\bh_t$ in \prettyref{eq:vector_moe} with second expert $g(A_2 x)$ replaced by a $2$-MoE, we can see from \prettyref{eq:grumoe} that GRU is a depth-$2$ hierarchical MoE. This is also illustrated in \prettyref{fig:gru_as_moe}.
\begin{figure}[t]
\centering
%\includegraphics[width=1.2\textwidth]{Presentation1.png}

\begin{tikzpicture}

\node[circle, draw=black, inner sep = 6.4 pt] at (-0.4,1.8) {};
\draw[->] (-0.4,2.1) -- (-0.4,2.7);
\node at (-0.3,3.0) {$y(x)=\bh_t$};

\filldraw[fill=blue!20!white, draw=black] (-2.3,0) -- (-1.0,0) -- (-1.0,1) -- (-2.3,1) -- cycle;
\node at (-1.6,0.5) {NN-1};


\node at (-1.9,-0.7) {$x=(\bx_t, \bh_{t-1})$};
\draw[->] (-1.6,-0.4)  -- (-1.6,0);



\node[circle, draw=black, inner sep=6pt] at (0.9,0.6) {};



\node at (-1.6 , 1.5) {$1-z_t$};
\draw[->] (-1.6,1)  -- (-0.7,1.6);

\node at (0.6  ,  1.4) {$z_t$};
\draw[->] (0.9,0.9)  -- (-0.1,1.6);


\filldraw[fill=blue!20!white, draw=black] (-0.6,-1.6) -- (0.7,-1.6) -- (0.7,-0.6) -- (-0.6,-0.6) -- cycle;
\node at (0.1,-1.1) {NN-2};

\node at (0.10,-2.3) {$x=(\bx_t, \bh_{t-1})$};
\draw[->] (0.05 , -2.0)  -- (0.05, -1.6);

\draw[->] (0.05,-0.6) -- (0.8,0.3) ;
\node at (0.0,0.0) {$1-r_t$};


\filldraw[fill=blue!20!white, draw=black] (2.2,-1.6) -- (3.5,-1.6) -- (3.5,-0.6) -- (2.2,-0.6) -- cycle;
\node at (2.9,-1.1) {NN-3};

\node at (2.90,-2.3) {$x=(\bx_t, \bh_{t-1})$};
\draw[->] (2.85 , -2.0)  -- (2.85, -1.6);



\draw[->] (2.85,-0.6) -- (1.1,0.4) ;
\node at (2.2,0.1) {$r_t$};

\node[draw,line width=1.0pt,color=orange,dotted,circle,inner ysep=15pt,fit={(-0.7,-1.1) (3.8,-1.1)}] {};

\end{tikzpicture}
\caption{GRU as a hierarchical $2$-MoE. The dotted circled portion indicates the canonical $2$-MoE in \prettyref{eq:k2moe}. NN-1, NN-2 and NN-3 denote specific input-output mappings obtained from \prettyref{eq:grumoe}. }
\label{fig:gru_as_moe}
\end{figure}


Note that in \prettyref{fig:gru_as_moe}, NN-1 models the mapping $(x_t,h_{t-1}) \mapsto h_{t-1}$, NN-2 represents $(x_t,h_{t-1}) \mapsto g(U_h x_{t})$, and NN-3 models $(x_t,h_{t-1}) \mapsto g(U_h x_t + W_h h_{t-1})$. Hence, this is slightly different from the traditional MoE setting in \prettyref{eq:kmoe} where the same activation $g(\cdot)$ is used for all the nodes. Nonetheless, we believe that studying this canonical model is a crucial first step which can shed important insights for a general setting.

==> Zipping for arXiv/introduction.tex <==
% !TEX root = gated_moe.tex
\section{Introduction}
In recent years, \emph{gated recurrent neural networks (RNNs)} such as LSTMs and GRUs have shown remarkable successes in a variety of challenging machine learning tasks such as machine translation, image captioning, image generation, hand writing generation, and speech recognition \citep{machinetranslation,imagecaption, speechrec,imagegen,handwritten}. A key interesting aspect and an important reason behind the success of these architectures is the presence of a \emph{gating mechanism} that dynamically controls the flow of the past information to the current state at each time instant. In addition, it is also well known that these gates prevent the vanishing (and exploding) gradient problem inherent to traditional RNNs \citep{hochreiter1997long}.

Surprisingly, despite their widespread popularity, there is very little theoretical understanding of these gated models. In fact, basic questions such as learnability of the parameters still remain open. Even for the simplest vanilla RNN architecture, this question was open until the very recent works of \cite{allen2018convergence} and \cite{allen2019can}, which provided the first theoretical guarantees of SGD for vanilla RNN models in the presence of non-linear activations. While this demonstrates that the theoretical analysis of these simpler models has itself been a challenging task, gated RNNs have an additional level of complexity in the form of gating mechanisms, which further enhances the difficulty of the problem. This motivates us to ask the following question:
\begin{question}
Given the complicated architectures of LSTMs/GRUs, can we find analytically tractable sub-structures of these models?
\end{question}

We believe that addressing the above question can provide new insights into a principled understanding of gated RNNs. In this paper, we make progress towards this and provide a positive answer to the question. In particular, we make a non-trivial connection that a GRU (gated recurrent unit) can be viewed as a time-series extension of a basic building block, known as \emph{Mixture-of-Experts (MoE)} \citep{JacJor,jor94}. In fact, much alike LSTMs/GRUs, MoE is itself a widely popular gated neural network architecture and has found success in a wide range of applications \citep{gpmoe,svmmoe,rasmussen2002infinite,YWG12,MaEb14,hmegp,deepmoe}. 
In recent years, there is also a growing interest in the fiels of natural language processing and computer vision to build complex neural networks incorporating MoE models to address challenging tasks such as machine translation \citep{gross2017hard, SMMD+17}. Hence the \emph{main goal} of this paper is to study MoE in close detail, especially with regards to learnability of its parameters.


The canonical MoE model is the following: Let $k \in \naturals$ denote the number of mixture components (or equivalently neurons). Let $\bx \in \reals^d$ be the input vector and $y \in \reals$ be the corresponding output. Then the relationship between $\bx$ and $y$ is given by: 
\begin{align}
y= \sum_{i=1}^k z_i \cdot g(\inner{\ba_i^\ast}{\bx}) + \xi, \quad \xi  \sim  \calN(0,\sigma^2),
\label{eq:kmoe}
\end{align}
where $g: \reals \to \reals$ is a non-linear activation function, $\xi$ is a Gaussian noise independent of $x$ and the latent Bernoulli random variable $z_i \in \{0,1\}$ indicates which expert has been chosen. In particular, only a single expert is active at any time, \ie $ \sum_{i=1}^k z_i =1$, and their probabilities are modeled by a soft-max function:
\begin{align*}
 \prob{z_i=1|\bx}=\frac{e^{\inner{\bw_i^\ast}{\bx}}}{\sum_{j=1}^k e^{\inner{\bw_j^\ast}{\bx}}}.
\end{align*}
Following the standard convention \citep{makkuva2018breaking,JacJor}, we refer to the vectors $\ba_i^\ast$ as \textit{regressors}, the vectors $\bw_i^\ast$ as either \textit{classifiers} or \textit{gating parameters}, and without loss of generality, we assume that $\bw_k^\ast=0$.
 
%Then the discriminative model $P_{y|\bx}$ for $k$-MoE is given by
%\begin{align*}
%P_{y|\bx} &= \sum_{i \in [k]} p_i^\ast(\bx) P_{y|\bx,i} =
% \sum_{i \in [k]} \frac{e^{\inner{\bw_i^\ast}{\bx}}}{\sum_{j \in [k]}e^{\inner{\bw_j^\ast}{\bx}}} \cdot \calN(y|g(\inner{\ba_i^\ast}{\bx}),\sigma^2).
%\end{align*}

%\begin{figure}[H]
%\label{fig:MoE}
%\centering
%
%\resizebox{40em}{16em}{
%
%\begin{tikzpicture}[domain=0:1.5,xscale=1,yscale=1]
%%\draw[->] (0,0)  -- (0,2.1) node[above] {\scriptsize $y$};
%%\draw[->] (0,0) -- (2.1,0) node[right] {\scriptsize $x$};
%
%%\node[draw] at (1.5,-2.5) {$\bx$};
%
%%\draw[-]  (1.5,-2.3)  -- (1.5,-1.7);
%
%%\draw[-] (1.5,-1.7)  -- (-4.0,-1.7);
%
%\draw[->] (-4.0,-1.7)  -- (-4.0,0.5);
%\node at (-4.0,-1.9)  {$\bx$};
%
%\draw[->] (-0.2,-1.7)  -- (-0.2,-0.5);
%\node at (-0.2,-1.9)  {$\bx$};
%
%%\draw[-] (1.5,-1.7)  -- (3.2,-1.7);
%
%\draw[->] (3.2,-1.7)  -- (3.2,-0.5);
%\node at (3.2,-1.9)  {$\bx$};
%
%%\draw[-] (3.2,-1.7)  -- (9.2,-1.7);
%
%\draw[->] (9.2,-1.7)  -- (9.2,-0.5);
%\node at (9.2,-1.9)  {$\bx$};
%
%\filldraw[fill=green!20!white, draw=black] (-1,-0.5) -- (1,-0.5) -- (1,0.5) -- (-1,0.5) -- cycle;
%\node at (-0.1,0.0) {$g(\inner{\ba_1^\ast}{\bx})$};
%\node at (-1.8,0.0) {Expert $1$};
%
%
%\filldraw[fill=green!20!white, draw=black] (2,-0.5) -- (4,-0.5) -- (4,0.5) -- (2,0.5) -- cycle;
%\node at (3.0,0.0) {$g(\inner{\ba_2^\ast}{\bx})$};
%\node at (4.8,0.0) {Expert $2$};
%
%\node at (6.6,0.0) {$\ldots$};
%
%
%
%\filldraw[fill=green!20!white, draw=black] (8,-0.5) -- (10,-0.5) -- (10,0.5) -- (8,0.5) -- cycle;
%\node at (9.0,0.0) {$g(\inner{\ba_k^\ast}{\bx})$};
%\node at (10.8,0.0) {Expert $k$};
%
%
%
%
%\draw[->] (0.0,0.5)  -- (5.3,3.3);
%\draw[->] (2.0,0.5)  -- (5.3,3.2);
%\draw[->] (9.0,0.5)  -- (5.7,3.2);
%
%%\node[draw] at (5.5,3.5) {y};
%
%\node[circle, draw=black, inner sep = 6.3 pt] at (5.5,3.5) {};
%\draw[->] (5.5,3.8) -- (5.5,4.1);
%\node at (5.5,4.3) {y};
%
%\filldraw[fill={rgb:orange,1;yellow,2;pink,5}, draw=black] (-3,0.5) -- (-5,0.5) -- (-5,2.5) -- (-3,2.5) -- cycle;
%\node[text width=2cm] at (-3.8,1.5) {Soft-max probability};
%\node[text width=3cm] at (-4.0,2.9) {Gating network};
%
%\draw[->] (-3,2.2)  -- (6.9,2.2);
%\draw[->] (-3,1.6)  -- (3.4,1.6);
%\draw[->] (-3,1.2)  -- (1.2,1.2);
%%\draw[->] (-3,0.8)  -- (2.2,0.8);
%
%\end{tikzpicture}
%}
%\caption{$k$-MoE architecture}
%\end{figure}

 Belying the canonical nature, and significant research effort, of the MoE model, the topic of learning MoE parameters is very poorly theoretically understood. In fact, the task of learning the parameters of a MoE, \ie $\ba_i^\ast$ and $\bw_i^\ast$, with provable guarantees is a long standing open problem for more than two decades \citep{SedghiA14a}. One of the key technical difficulties is that in a MoE, there is an inherent \emph{coupling} between the regressors $a_i^\ast$ and the gating parameters $w_i^\ast$, as can be seen from \prettyref{eq:kmoe}, which makes the problem challenging \citep{ho2019convergence}. In a recent work \citep{makkuva2018breaking}, the authors provided the first consistent algorithms for learning MoE parameters with theoretical guarantees. In order to tackle the aforementioned coupling issue, they proposed a clever scheme to first estimate the regressor parameters $\ba_i^\ast$ and then estimating the gating parameters $\bw_i^\ast$ using a combination of spectral methods and the EM algorithm. However, a major draw back is that this approach requires specially crafted algorithms for learning each of these two sets of parameters. In addition, they lack finite sample guarantees. Since SGD and its variants remain the de facto algorithms for training neural networks because of their practical advantages, and inspired by the successes of these gradient-descent based algorithms in finding global minima in a variety of non-convex problems, we ask the following question:
 
%  In the absence of the gating parameters, MoE reduces to the well-studied \emph{mixtures of generalized linear models (GLMs)}, which are typically learnt using spectral methods \cite{SedghiA14a,zhong16glm,YCS16}. However, none of the existing techniques for GLMs generalize since the presence of the gating parameters significantly complicates the super symmetric tensor structure needed for these tensor based methods. Another common approach to learn the parameters is to use a $l_2$ loss function,
%\begin{align}
%L_2(\bA,\bW) = \Expect[\|\hat{y}-y\|^2], \quad \hat{y}= \sum_{i \in [k]}p_i(\bx)g(\inner{\ba_i}{\bx}),
%\label{eq:l2}
%\end{align} 
%which is prone to bad local minima as demonstrated empirically in the original work of \cite{JacJor} (which we verify in our experiments too), which also emphasized the importance of the right objective function to learn the parameters. Moreover, the work-horse of parameter learning in latent variable models, the EM algorithm, is also prone to bad local minima as established in \cite{makkuva2018breaking}. This motivates us to ask the following question:

\begin{question}
How do we design objective functions amenable to efficient optimization techniques, such as SGD, with provable learning guarantees for MoE?
\end{question}

In this paper, we address this question in a principled manner and propose two non-trivial non-convex loss functions $L_4(\cdot)$ and $L_{\log}(\cdot)$ to learn the regressors and the gating parameters respectively. In particular, our loss functions possess nice landscape properties such as local minima being global and the global minima corresponding to the ground truth parameters. We also show that gradient descent on our losses can recover the true parameters with \emph{global/random initializations}. To the best of our knowledge, ours is the first GD based approach with finite sample guarantees to learn the parameters of MoE. While our procedure to learn $\{a_i^\ast\}$ and $\{w_i^\ast\}$ separately and the technical assumptions are similar in spirit to \cite{makkuva2018breaking}, our loss function based approach with provable guarantees for SGD is significantly different from that of \cite{makkuva2018breaking}. We summarize our main contributions below:

\begin{itemize}
\item \textbf{MoE as a building block for GRU:} We provide the first connection that the well-known GRU models are composed of basic building blocks, known as MoE. This link provides important insights into theoretical understanding of GRUs and further highlights the importance of MoE.

\item \textbf{Optimization landscape design with desirable properties:} We design \emph{two non-trivial} loss functions $L_4(\cdot)$ and $L_{\log}(\cdot)$ to learn the regressors and the gating parameters of a MoE separately. We show that our loss functions have nice landscape properties and are amenable to simple local-search algorithms. In particular, we show that SGD on our novel loss functions recovers the parameters with \emph{global/random} initializations.
\item \textbf{First sample complexity results:} We also provide the first sample complexity results for MoE. We show that our algorithms can recover the true parameters with accuracy $\varepsilon$ and with high probability, when provided with samples \emph{polynomial} in the dimension $d$ and $1/\varepsilon$. 
\end{itemize}

%\textbf{(i) Separate estimation of regressors and gating parameters.} We propose a strategy to learn the regressors and the gating parameters \emph{separately} with provable recoverable guarantees, taking into account the modular structure inherent to the problem. In fact, the traditional approach of using the same loss function to learn both the set of parameters jointly suffers from bad optima \cite{JacJor}. 
%To the best of our knowledge, this is the first work that highlights the role of parameter decoupling in learning the parameters with global initializations.

%\textbf{(ii) Novel non-convex loss functions design.}
%We design \emph{two non-trivial} loss functions $L_4(\cdot)$ and $L_{\log}$ to learn the regressors and the gating functions separately. We show that our loss functions have nice landscape properties. For example, all local minima are global minima and global minima correspond to the ground truth parameters. Thus our loss functions are amenable to efficient optimization algorithms.
%
%\textbf{(iii) First provable guarantees for GD.} In this paper, we provide the first gradient descent based algorithm to learn the true parameters of a MoE. In particular, we show that GD on our novel loss functions recovers the parameters with \emph{global/random} initializations. It is important to note that there are only a handful of models where the parameters can be learnt through global initializations, such as mixtures of two symmetric Gaussians \cite{Daskalakis17,hsulengthy}, and it is quite remarkable that a simple algorithm like GD can learn the parameters with any random initialization. 
%
%\textbf{(iv) First sample complexity results.} In addition, we also provide the first sample complexity results for MoE. We show that our algorithms can recover the true parameters with accuracy $\varepsilon$ when provided with samples \emph{polynomial} in dimension and $1/\varepsilon$ with high probability. 

%\begin{figure}[h]
%\centering
%\resizebox{26em}{12em}{
%\begin{tikzpicture}%[transform canvas={scale=0.9}]
%
%
%\filldraw[fill=red!20!white, draw=black] (-2.5,1.0) -- (-4.8,1.0) -- (-4.8,2.0) -- (-2.5,2.0) -- cycle;
%\node[text width=2cm] at (-2.8,1.5) {$L_4$};
%\node at (-3.5,2.5) {$4$-order tensor loss};
%\draw[->] (-2.5,1.5) -- (-1.5,1.5) ;
%\node at (0.4,1.5) {Regressors $\{\hat{\ba}_1,\ldots,\hat{\ba}_k \}$};
%
%\filldraw[fill=red!20!white, draw=black] (-2.5,-1.0) -- (-4.8,-1.0) -- (-4.8,-2.0) -- (-2.5,-2.0) -- cycle;
%\node[text width=2cm] at (-2.8,-1.5) {$L_{\mathrm{\log}}$};
%\node at (-3.3,-2.5) {Log-likelihood loss};
%\draw[->] (-2.5,-1.5) -- (-1.5,-1.5) ;
%\node at (0.4,-1.5) {Classifiers $\{\hat{\bw}_1,\ldots,\hat{\bw}_k \}$};
%
%
%\draw[->] (0.8,1.2) -- (-3.5,-1.0);
%
%\filldraw[fill=blue!20!white, draw=black] (-6.0,1.2) -- (-9.0,1.2) -- (-9.0,0.0) -- (-6.0,0.0) -- cycle;
%\node at (-7.5,0.8) {Quartic \& Quadratic };
%\node at (-7.5,0.4) {Transform };
%\draw[->] (-6.0,0.6) -- (-4.8,1.4) ;
%
%
%\filldraw[fill=blue!20!white, draw=black] (-6.0,3.2) -- (-9.0,3.2) -- (-9.0,2.0) -- (-6.0,2.0) -- cycle;
%\node at (-7.5,2.6) {Score function};
%\draw[->] (-6.0,2.6) -- (-4.8,1.6) ;
%
%
%\filldraw[fill=white, draw=black] (-10.0,3.2) -- (-11.0,3.2) -- (-11.0,0.0) -- (-10.0,0.0) -- cycle;
%\node at (-10.5,3.5) {Samples};
%\node at (-10.5,2.6) {$\bx$};
%\draw[->] (-10.0,2.6) -- (-9.0,2.6);
%
%\node at (-10.5,0.6) {$y$};
%\draw[->] (-10.0,0.6) -- (-9.0,0.6);
%
%
%\draw (-10.5,0.0) -- (-10.5,-1.5);
%\draw[->] (-10.5,-1.5) -- (-4.8,-1.5);
%
%
%
%%\draw[->] (-3.5,1.0)  -- (-3.5,0.4);
%%\node at (-3.5,0.0) {$\hat{\ba}_1,\hat{\ba}_2$};
%%
%%
%%\filldraw[fill=red!20!white, draw=black] (0.0,1.0) -- (-1.3,1.0) -- (-1.3,2.0) -- (0.0,2.0) -- cycle;
%%\node[text width=2cm] at (0.2,1.5) {$L_{\mathrm{\log}}$};
%%\node at (1.4,1.5) {Log-likelihood};
%%
%%
%%\draw[->] (-0.5,1.0)  -- (-0.5,0.4);
%%\node at (-0.5,0.0) {$\hat{\bw}$};
%
%
%
%
%
%\end{tikzpicture}
%}
%\caption{Algorithm to learn the MoE parameters: (a) First we take non-linear transformations on the samples $(\bx_i,y_i)$ to compute the tensor based loss $L_4$, (b) SGD on $L_4$ recovers the regressors, (c) The loss $L_{\mathrm{\log}}$ uses the learnt regressors and samples to learn the gating parameters through gradient descent. }
%\label{fig:scheme}
%\end{figure}
%
%{\em Novelty:} The aforementioned contributions are driven by the following key technical innovations:
%
%\textbf{Quartic and Quadratic Transforms for outputs.} The notion of score transformation for input $\bx$ is one of the key techniques behind parameter recovery in mixtures of GLMs \cite{scorebusiness,SedghiA14a,zhong16glm}. The basic idea is to construct a \emph{super symmetric tensor} and to use tensor decomposition algorithms to learn the parameters. However, these methods significantly rely on the fact that the mixing probabilities are constant and break down in the context of MoEs because of the presence of gating parameters. In this paper, we address this challenge and introduce a novel notion of ``Quartic and Quadratic Transforms (QQT)" for processing the outputs.
%
%We show that the carefully designed QQT on the outputs together with the score transformations on the input yield a super symmetric tensor for MoE (\prettyref{thm:fourthtensor}). The QQT are specific to the choice of non-linearity $g$ and the noise variance $\sigma$. In fact, for the special case of $g=\mathrm{linear}$ and $\sigma=0$, these transforms are exactly the $4^{\mathrm{th}}$ and $2^{\mathrm{nd}}$ Hermite polynomials. It is a well known fact that Hermite polynomials are orthogonal under Gaussian measure, \ie $\Expect_{Z \sim \calN(0,1)}[H_m(Z)H_n(Z)]=\delta_{mn}$ \cite{hermitestuff}. We make an interesting connection of this fact with super-symmetric tensor construction via Stein's lemma. Moreover, we generalize this approach to deal with a wide class of non-linearities including $\mathrm{linear},\mathrm{sigmod}$ and $\mathrm{ReLU}$.
%Finally, beyond the obvious applications, this paper opens up a new realm of utilizing different loss functions for different sets of parameters, for example, for learning multiple layers in a neural network. 



\textbf{Related work.}
Linear dynamical systems can be thought of as the linear version of RNNs. There is a huge literature on the topic of learning these linear systems \cite{alaeddini2018linear,arora2018towards,dean2017sample, dean2018safely, marecek2018robust, oymak2018non, simchowitz2018learning,hardt2018gradient}. However these works are very specific to the linear setting and do not extend to non-linear RNNs. \cite{allen2018convergence} and \cite{allen2019can} are two recent works to provide first theoretical guarantees for learning RNNs with ReLU activation function. However, it is unclear how these techniques generalize to the gated architectures. In this paper, we focus on the learnability of MoE, which are the building blocks for these gated models. 

While there is a huge body of work on MoEs (see \cite{YWG12,MaEb14} for a detailed survey), the topic of learning MoE parameters is theoretically less understood with very few works on it. \cite{emmoeanalysis} is one of the early works that showed the local convergence of EM.  In a recent work, \cite{makkuva2018breaking} provided the first consistent algorithms for MoE in the population setting using a combination of spectral methods and EM algorithm. However, they do not provide any finite sample complexity bounds. In this work, we provide a unified approach using GD to learn the parameters with finite sample guarantees. To the best of our knowledge, we give the first gradient-descent based method with consistent learning guarantees, as well as the first finite-sample guarantee for any algorithm. The topic of designing the loss functions and analyzing their landscapes is a hot research topic in a wide variety of machine learning problems: neural networks \citep{identitymatters,kawa,reluanalysis,electron_proton,dhillon, landscapedesign,gao2018learning}, matrix completion \citep{bhoja}, community detection \citep{bandeira}, orthogonal tensor decomposition \citep{escapesaddle}. In this work, we present the first objective function design and the landscape analysis for MoE. 

\textbf{Notation.} We denote $\ell_2$-Euclidean norm by $\norm{\cdot}$. $[d] \define \{1,2,\ldots,d\}$. $\{e_i\}_{i=1}^d$ denotes the standard basis vectors in $\reals^d$. We denote matrices by capital letters like $A,W$, etc. For any two vectors $x,y \in \reals^d$, we denote their Hadamard product by $x \odot y$. $\sigma(\cdot)$ denotes the sigmoid function $\sigma(z)=1/(1+e^{-z}),z \in \reals$. For any $z=(z_1,\ldots,z_k) \in \reals^k$, $\mathrm{softmax}_i(z)=\exp(z_i)/(\sum_j \exp(z_j))$. $\calN(mu,\Sigma)$ denotes the Gaussian distribution with mean $\mu \in \reals^d$ and covariance $\Sigma \in \reals^{d\times d}$. Through out the paper, we interchangeably denote regressors as $\{a_i\}$ or $A$, and gating parameters as $\{w_i\}$ or $W$.

{\bf Overview.} The rest of the paper is organized as follows: In \prettyref{sec:connection}, we establish the precise mathematical connection between the well known GRU model and the MoE model. Building upon this correspondence, which highlights the importance of MoE, in \prettyref{sec:optim_landscape} we design two novel loss functions to learn the respective regressors and gating parameters of a MoE and present our theoretical guarantees. In \prettyref{sec:experiments}, we empirically validate that our proposed losses perform much better than the current approaches on a variety of settings. 

%We denote the scalars with lower case letters like $y$, Euclidean vectors by bold face lower case letters like $\bx$, and matrices by capital letters $\bA$. $\bx^{\otimes 4}=\bx \otimes \bx \otimes \bx \otimes \bx$ denotes the fourth-order tensor product of $\bx$. $\sym(\ba \otimes \bb \otimes \ba \otimes \bb)$ denotes the symmetrized version of $\ba \otimes \bb \otimes \ba \otimes \bb$ where we add all possible permutations of the indices. 

==> Zipping for arXiv/optimization_landscape.tex <==
% !TEX root = gated_moe.tex
\section{Optimization landscape design for MoE}
\label{sec:optim_landscape}
In the previous section, we presented the mathematical connection between the GRU and the MoE. In this section, we focus on the learnability of the MoE model and design two novel loss functions for learning the regressors and the gating parameters separately.
%and present our theoretical guarantees.
%In \prettyref{sec:L_4}, we define a new regressor loss $L_4$ and present our theoretical results. In \prettyref{sec:gradgating}, we present the gating loss $L_{\mathrm{log}}$ followed by our theoretical guarantees.

\subsection{Loss function for regressors: $L_4$}
\label{sec:L_4}

To motivate the need for loss function design in a MoE, first we take a moment to highlight the issues with the traditional approach of using the mean square loss $\ell_2$. If $(x,y)$ are generated according to the ground-truth MoE model in \prettyref{eq:kmoe}, $\ell_2(\cdot)$ computes the quadratic cost between the expected predictions $\hat{y}$ and the ground-truth $y$, \ie
\begin{align*}
\ell_2(\{a_i\}, \{w_i\}) = \Expect_{(x,y)}\|\hat{y}(x)-y\|^2,
\label{eq:l2_loss}
\end{align*} 
where $\hat{y}(x)= \sum_{i} \mathrm{softmax}_i(w_1^\top x, \ldots, w_{k-1}^\top x,0)~g(\ba_i^\top \bx)$ is the predicted output, and $\{a_i \},\{w_i\}$ denote the respective regressors and gating parameters. It is well-known that this mean square loss is prone to bad local minima as demonstrated empirically in the earliest work of \cite{JacJor} (we verify this in \prettyref{sec:experiments} too), which also emphasized the importance of the right objective function to learn the parameters. Note that the bad landscape of $\ell_2$ is not just unique to MoE, but also widely observed in the context of training neural network parameters \citep{livni2014computational}. In the one-hidden-layer NN setting, some recent works \citep{landscapedesign, gao2018learning} addressed this issue by designing new loss functions with good landscape properties so that standard algorithms like SGD can provably learn the parameters. However these methods do not generalize to the MoE setting since they crucially rely on the fact that the coefficients $z_i$ appearing in front of the activation terms $g(\inner{a_i^\ast}{x})$ in \prettyref{eq:kmoe}, which correspond to the linear layer weights in NN, are constant. Such an assumption does not hold in the context of MoEs because the gating probabilities depend on $x$ in a parametric way through the softmax function and hence introducing the coupling between $w_i^\ast$ and $a_i^\ast$ (a similar observation was noted in \cite{makkuva2018breaking} in the context of spectral methods).


%However, the mean square error $\ell_2$ does not respect this modular structure and learning these two different sets of parameters jointly through SGD entangles them in a complicated manner leading to bad minima. Can we design loss functions adhering to this special structure inherent to MoE?
%
%common joint-loss function approaches. Observe from \prettyref{eq:kmoe} that the parameters $\bw_i^\ast$ and $\ba_i^\ast$ play different roles in generating the data: $\bw_i^\ast$ are used for multi-class classification whereas $\ba_i^\ast$ for regression.
%
%We answer this question precisely through construction of a $4^{\mathrm{th}}$ and $2^{\mathrm{nd}}$-order super symmetric tensors involving \emph{just} the regressors $\ba_i^\ast$ (see \prettyref{thm:fourthtensor}) and constructing a loss function using its projections along the parameter space. While the traditional approach to construct such tensors involve forming the cross moments between the input $\bx$ and the output $y$ in mixtures of GLMs, the inherent coupling between $\ba_i^\ast$ and $\bw_i^\ast$ in a MoE complicates these moments, rendering these techniques ineffective (see Proof of \prettyref{thm:fourthtensor}). 

In order to address the aforementioned issues, inspired by the works of \cite{landscapedesign} and \cite{gao2018learning}, we design a novel loss function $L_4(\cdot)$ to learn the regressors first. Our loss function depends on two distinct special transformations on both the input $x \in \reals^d$ and the output $y \in \reals$. For the output, we consider the following transformations:
%``Quartic and Quadratic Transform (QQT)" for the output $y$, \ie
\begin{align}
\calQ_4(y) \define y^4+\alpha y^3+ \beta y^2+ \gamma y, \hspace{0.4em} \calQ_2(y) \define y^2+ \delta y,
\end{align}
where the set of coefficients $(\alpha,\beta,\gamma,\delta)$ are dependent on the choice of non-linearity $g$ and noise variance $\sigma^2$.  These are obtained by solving a simple linear system (see \prettyref{app:non_linearclass}). For the special case $g=\Id$, which corresponds to linear activations, the Quartic transform is $\calQ_4(y)=y^4-6y^2(1+\sigma^2)+3+3\sigma^4-6\sigma^2$ and the Quadratic transform is $\calQ_2(y)=y^2-(1+\sigma^2)$. For the input $\bx$, we assume that $ x \sim \calN(0,I_d)$, and for any two fixed $u,v \in \reals^d$, we consider the projections of multivariate-Hermite polynomials \cite{grad1949note,holmquist1996d, scorebusiness} along these two vectors, \ie
\begin{align*}
t_3(\bu,\bx) &= \frac{(\bu^\top \bx)^2 - \norm{\bu}^2}{c'_{g,\sigma}}, \\
t_2(\bu, \bx) &= \frac{(\bu^\top \bx)^4 - 6 \norm{\bu}^2 (\bu^\top \bx)^2 + 3\norm{\bu}^4}{c_{g,\sigma}},\\
t_1(\bu, \bv ,\bx) &=((\bu^\top \bx)^2(\bv^\top \bx)^2 - \norm{\bu}^2(\bv^\top \bx)^2 \\
& \hspace{1.0em}- 4(\bu^\top \bx)(\bv^\top \bx)(\bu^\top \bv) - \norm{\bv}^2 (\bu^\top \bx)^2\\
& \hspace{1.0em} +\norm{\bu}^2 \norm{\bv}^2+ 2 (\bu^\top \bv)^2)/c_{g,\sigma},
\end{align*}
where $c_{g,\sigma}$ and $c'_{g,\sigma}$ are two non-zero constants depending on $g$ and $\sigma$. These transformations $(t_1, t_2, t_3)$ on the input $x$ and $(\calQ_4, \calQ_2)$ on the output $y$ can be viewed as extractors of higher order information from the data. The utility of these transformations is concretized in \prettyref{thm:landscape} through the loss function defined below.
%we use the traditional score funcions \cite{scorebusiness}:
%\begin{align}
%\calS_m(\bx) \define (-1)^m \frac{\nabla_{\bx}^{(m)}f(\bx)}{f(\bx)}, \quad f \text{ is the pdf of } \bx.
%\end{align}
%In this paper we focus on $m=2,4$. When $\bx \sim \calN(0,\bI_d)$, we know that $\calS_2(\bx) = \bx \otimes \bx - \bI$ and
%\begin{align*}
%\calS_4(\bx) = \bx^{\otimes 4}-\sum_{i \in [d]} \sym\pth{\bx \otimes \be_i \otimes \be_i \otimes \bx }+\sum_{i,j} \sym \pth{\be_i \otimes \be_i \otimes \be_j \otimes \be_j}.
%\end{align*}
%The score transformations $\calS_4(\bx)$ and $\calS_2(\bx)$ can be viewed as multi-variate polynomials in $\bx$ of degrees $4$ and $2$ respectively. In fact, they are the multi-variate Hermite polynomials. These transformations can be viewed as extractors of higher order information from the training data. The utility of these transformations is concretized in \prettyref{thm:fourthtensor}. First we formally state our assumptions for the theoretical results.
%
%\begin{assumption}\normalfont
%\label{assump:setassump}
%\begin{enumerate}
%\item $\bx$ follows a standard Gaussian distribution, \ie $\bx \sim \calN(0,\bI_d)$.
%\item $\norm{\ba_i^\ast}=1$ for all $i \in [k]$ and $\norm{\bw_i^\ast} \leq R$ for all $i \in [k-1]$.
%\item The regressors $\ba_1^\ast,\ldots,\ba_k^\ast$ are linearly independent and the classifiers $\{\bw_i^\ast\}_{i \in [k-1]}$ are orthogonal to the span $\calS=\mathrm{span}\sth{\ba_1^\ast,\ldots,\ba_k^\ast}$, and $2k-1 < d$.
%\item The non-linearity $g: \reals \to \reals$ is $(\alpha,\beta,\gamma,\delta)-\valid$, which we define in \prettyref{app:non_linearclass}. For example, this class includes the popular choices of linear, sigmoid and ReLU activation functions.
%\end{enumerate}
%\end{assumption}
%
%\begin{theorem}[Super symmetric tensor construction]
%\label{thm:fourthtensor}
%Let $(\bx,y)$ be generated according to \prettyref{eq:kmoe} and that \prettyref{assump:setassump} holds. Then
%\begin{align*}
%\calT_4 \define \Expect[\calQ_4(y) \cdot \calS_4(\bx)]&= c_{g,\sigma} \sum_{i \in [k]}\Expect[p_i^\ast(\bx)] \cdot \ba_i^\ast \otimes \ba_i^\ast \otimes \ba_i^\ast \otimes \ba_i^\ast,\\
%\calT_2 \define \Expect[\calQ_2(y) \cdot \calS_2(\bx)] &=c'_{g,\sigma} \sum_{i \in [k]}\Expect[p_i^\ast(\bx)] \cdot \ba_i^\ast \otimes \ba_i^\ast,
%\end{align*}
%where $c_{g,\sigma}$ and $c'_{g,\sigma}$ are two non-zero constants depending on $g$ and $\sigma$.
%\end{theorem}
%\begin{remark}\normalfont
%We found empirically that the orthogonality assumption is only needed for the theoretical results whereas our algorithms still work in the relaxed setting (see \prettyref{app:non_orthogonal} for experiments).
%\end{remark}
%\begin{hproof}For the sake of expositional ease, let $g$ be the linear function. Then we have that $
%\Expect[y|\bx] = \sum_{i \in [k]} p_i^\ast(\bx) \inner{\ba_i^\ast}{\bx}$.
%Using the generalized Stein's lemma \cite{scorebusiness}, we get that
%\begin{align*}
%\Expect[y \cdot \calS_4(\bx)]= \sum_{i \in [k]}\Expect[p_i^\ast(\bx) \inner{\ba_i^\ast}{\bx} \cdot \calS_4(\bx)]=\sum_{i \in [k]}\Expect[\nabla_{\bx}^{(4)}(p_i^\ast(\bx) \inner{\ba_i^\ast}{\bx})].
%\end{align*}
%Since $p_i^\ast(\bx)$ depends on all the gating parameters $\bw_1^\ast,\ldots,\bw_{k-1}^\ast$, it is easy to see from the chain-rule for multi-derivatives that the fourth-order tensor $\Expect[\nabla_{\bx}^{(4)}(p_i^\ast(\bx) \inner{\ba_i^\ast}{\bx})]$ will contain all fourth order rank $1$-terms involving the tensor product of $\bw_1^\ast,\ldots,\bw_{k-1}^\ast$ and $\ba_i^\ast$ for any fixed $i$. Notice that this issue is not present in the context of mixtures of GLMs \cite{SedghiA14a} since $p_i^\ast(\bx)$ is a constant in that setting. In order to circumvent this, we consider a quartic transformation $\calQ_4(y)=y^4-6y^2(1+\sigma^2)+3+3\sigma^4-6\sigma^2$ and obtain that
%\begin{align*}
%\Expect[\calQ_4(y)|\bx]=\sum_{i \in [k]} p_i^\ast(\bx) (\inner{\ba_i^\ast}{\bx}^4-6\inner{\ba_i^\ast}{\bx}^2+3).
%\end{align*}
%Now it turns out that after using the orthogonality of $\bw_i^\ast$ and $\ba_i^\ast$, and the fact $\Expect[p(Z)]=\Expect[p'(Z)]=\Expect[p''(Z)]=\Expect[p'''(Z)]=0$ for fourth-Hermite polynomial $p(z)=z^4-6z^2+3$ and $Z \sim \calN(0,1)$, we can nullify the cross-moments between $\bw_i^\ast$'s and $\ba_i^\ast$'s to obtain that
%\begin{align*}
%\Expect[\calQ_4(y)\cdot \calS_4(\bx)]=24\sum_{i \in [k]}\Expect[p_i^\ast(\bx)]. (\ba_i^\ast)^{\otimes 4}.
%\end{align*}
%These observations can be generalized to non-linear choices of $g$ and also for the second-order score functions, which are more technical in detail  and we describe them in \prettyref{app:non_linearclass}.
%\end{hproof}
%In order to construct our tensor based loss, for any fixed $\bu, \bv \in \reals^d$, we define the functions $t_1,t_2$ and $t_3$ which are the projections of our score transformations along these directions, \ie
%\begin{align*}
%t_1(\bu, \bv ,\bx) \define \frac{\calS_4(\bx)(\bu,\bu,\bv,\bv)}{c_{g,\sigma}}, \quad t_2 (\bu, \bx)  \define \frac{\calS_4(\bx)(\bu,\bu,\bu,\bu)}{c_{g,\sigma}}, \quad t_3(\bu,\bx) \define \frac{\calS_2(\bx)(\bu,\bu)}{c'_{g,\sigma}}.
%\end{align*}
%Using the expressions for $\calS_2(\bx)$ and $\calS_4(\bx)$, we know that
Denoting the set of our regression parameters by the matrix $\bA^\top= [\ba_1|\ba_2|\ldots|\ba_k] \in \reals^{d \times k}$, we now define our objective function $L_4(\bA)$ as
\begin{align}
&L_4(\bA) \nonumber \\
&\define \sum_{\substack{i,j \in [k] \\i \neq j}} \Expect[\calQ_4(y) t_1(\ba_i,\ba_j,\bx)] - \mu \sum_{i \in [k]} \Expect[\calQ_4(y) t_2(\ba_i,\bx)] \nonumber \\  
& + \lambda \sum_{i \in [k]} \pth{\Expect[\calQ_2(y) t_3(\ba_i,\bx)]-1}^2
+\frac{\delta}{2} \norm{\bA}_F^2,
\label{eq:tensorloss}
\end{align}
where $\mu,\lambda, \delta>0$ are some positive regularization constants. Notice that $L_4$ is defined as an expectation of terms involving the data transformations: $\calQ_4, \calQ_2, t_1, t_2,$ and $t_3$. Hence its gradients can be readily computed from finite samples and is amenable to standard optimization methods such as SGD for learning the parameters. Moreover, the following theorem highlights that the landscape of $L_4$ does not have any spurious local minima.

%Notice that the loss $L$ is a fourth-order polynomial in our parameters $\bA$ and the data $(\bx,y)$.

\begin{theorem}[Landscape analysis for learning regressors]
\label{thm:landscape}
Under the mild technical assumptions of \cite{makkuva2018breaking}, the loss function $L_4$ does not have any spurious local minima. More concretely, let $\varepsilon>0$ be a given error tolerance. Then we can choose the regularization constants $\mu,\lambda$ and the parameters $\varepsilon,\tau$ such that if $A$ satisfies
\begin{align*}
\norm{\nabla L_4(\bA)}_2 \leq \varepsilon, \quad \nabla^2 L_4(\bA) \succcurlyeq  -\tau/2,
\end{align*}
then $(\bA^\dagger)^\top=   \bP \bD \Gamma \bA^\ast+ \bE$, where $\bD$ is a diagonal matrix with entries close to $1$, $\Gamma$ is a diagonal matrix with $\Gamma_{ii}=\sqrt{\Expect[p_i^\ast(\bx)]}$, $\bP$ is a permutation matrix and $\norm{\bE} \leq \varepsilon_0$. Hence every approximate local minimum is $\varepsilon$-close to the global minimum. 
\end{theorem}

\textbf{Intuitions behind the theorem and the special transforms:} While the transformations and the loss $L_4$ defined above may appear non-intuitive at first, the key observation is that $L_4$ can be viewed as a fourth-order polynomial loss in the parameter space, \ie
\begin{align}
&L_4(\bA) \nonumber \\
 & = \sum_{m \in [k]} \Expect[p_m^\ast(\bx)] \sum_{\substack{i \neq j \\ i,j \in [k]}} \inner{\ba_m^\ast}{\ba_i}^2 \inner{\ba_m^\ast}{\ba_j}^2 \nonumber \\
 & - \mu \sum_{m,i \in [k]} \Expect[p_m^\ast(\bx)] \inner{\ba_m^\ast}{\ba_i}^4   \label{eq:alternate} \\
& +\lambda \sum_{i \in [k]} (\sum_{m \in [k]} \Expect[p_m^\ast(\bx)] \inner{\ba^\ast_m}{\ba_i}^2-1)^2 +  \frac{\delta}{2} \norm{\bA}_F^2 \nonumber,
\end{align}
where $p_i^\ast$ refers to the softmax probability for the $i^{th}$ label with true gating parameters, \ie $p_i^\ast(x)=\mathrm{softmax}_i(\inner{w_1^\ast}{x},\ldots,\inner{w_{k-1}^\ast}{x},0)$. This alternate characterization of $L_4(\cdot)$ in \prettyref{eq:alternate} is the crucial step towards proving \prettyref{thm:landscape}. Hence these specially designed transformations on the data $(x,y)$ help us to achieve this objective. Given this viewpoint, we utilize tools from \cite{landscapedesign}, where a similar loss involving fourth-order polynomials were analyzed in the context of $1$-layer ReLU network, to prove the desired landscape properties for $L_4$. The full details behind the proof are provided in \prettyref{app:proofregressor}. Moreover, in \prettyref{sec:experiments} we empirically verify that the technical assumptions are only needed for the theoretical results and that our algorithms are robust to these assumptions, and work equally well even when we relax them.
%\begin{hproof} The crucial step in analyzing the landscape of $L$ is to give an alternative characterization for it in the form of
%\begin{align}
%L_4(\bA) &= \sum_{m \in [k]} \Expect[p_m^\ast(\bx)] \sum_{\substack{i \neq j \\ i,j \in [k]}} \inner{\ba_m^\ast}{\ba_i}^2 \inner{\ba_m^\ast}{\ba_j}^2 - \mu \sum_{m,i \in [k]} \Expect[p_m^\ast(\bx)] \inner{\ba_m^\ast}{\ba_i}^4 \nonumber \\
%&\hspace{3em} +\lambda \sum_{i \in [k]} (\sum_{m \in [k]} \Expect[p_m^\ast(\bx)] \inner{\ba^\ast_m}{\ba_i}^2-1)^2 +  \frac{\delta}{2} \norm{\bA}_F^2. \label{eq:alternate}
%\end{align}
%We can prove \prettyref{eq:alternate} using the tensor structure of $\calT_4,\calT_2$ and the definitions of $t_1,t_2$ and $t_3$. We can notice that $L$ is a fourth-order polynomial in our parameters $\bA$. Now we use the techniques from \cite{landscapedesign}, where the authors analyzed a similar tensor based loss for learning a $1$-layer ReLU network, to characterize the landscape of $L$ in our setting. We provide the full details in .
%\end{hproof}

In the finite sample regime, we replace the population expectations in \prettyref{eq:tensorloss} with sample average to obtain the empirical loss $\hat{L}$.  The following theorem establishes that $\hat{L}$ too inherits the same landscape properties of $L$ when provided enough samples.

%\begin{align*}
%\hat{L}(\bA) \define \sum_{\substack{i,j \in [k] \\i \neq j}} \hat{\Expect}[\calQ_4(y) t_1(\ba_i,\ba_j,\bx)] - \mu \sum_{i \in [k]} \hat{\Expect}[\calQ_4(y) t_2(\ba_i,\bx)] + \lambda \sum_{i \in [k]} \pth{ \hat{\Expect}[\calQ_2(y) t_3(\ba_i,\bx)]-1}^2+\frac{\delta}{2} \norm{\bA}_F^2,
%\end{align*}
%where $\hat{\Expect}$ refers to the empirical expectation with respect to the \iid samples $\{(\bx_i,y_i)\}_{i=1}^n$. The following theorem establishes that $\hat{L}$ too inherits the same landscape properties of $L$ when provided enough samples.
\begin{theorem}[Finite sample landscape]
\label{thm:finitelandscape}
There exists a polynomial $\mathrm{poly}(d,1/\varepsilon)$ such that whenever $n \geq \mathrm{poly}(d,1/\varepsilon)$, $\hat{L}$ inherits the same landscape properties as that of $L$ established in \prettyref{thm:landscape} with high probability. Hence stochastic gradient descent on $\hat{L}$ converges to an approximate local minima which is also close to a global minimum in time polynomial in $d,1/\varepsilon$.
\end{theorem}
\begin{remark}\normalfont
Notice that the parameters $\{\ba_i\}$ learnt through SGD are some permutation of the true parameters $\ba_i^\ast$ upto sign flips. This sign ambiguity can be resolved using existing standard procedures such as Algorithm 1 in \cite{landscapedesign}. In the remainder of the paper, we assume that we know the regressors upto some error $\varepsilon_{\mathrm{reg}}>0$ in the following sense: $\max_{i \in [k]}\norm{a_i-a_i^\ast}=\sigma^2 \varepsilon_{\mathrm{reg}}$.
\end{remark}

\subsection{Loss function for gating parameters: $L_{\log}$}
\label{sec:gradgating}

In the previous section, we have established that we can learn the regressors $\ba_i^\ast$ upto small error using SGD on the loss function $L_4$. Now we are interested in answering the following question: Can we design a loss function amenable to efficient optimization algorithms such as SGD with recoverable guarantees to learn the gating parameters? 

In order to gain some intuition towards addressing this question, consider the simplified setting of $\sigma=0$ and $\bA=\bA^\ast$. In this setting, we can see from \prettyref{eq:kmoe} that the output $y$ equals one of the activation values $g(\inner{\ba_i^\ast}{\bx})$, for $i \in [k]$, with probability $1$. Since we already have access to the true parameters, \ie $A=\bA^\ast$, we can see that we can exactly recover the hidden latent variable $z$, which corresponds to the chosen hidden expert for each sample $(\bx,y)$. Thus the problem of learning the \textit{classifiers} $\bw_i^\ast,\ldots,\bw_{k-1}^\ast$ reduces to a multi-class classification problem with label $z$ for each input $\bx$ and hence can be efficiently solved by traditional methods such as logistic regression. It turns out that these observations can be formalized to deal with more general settings (where we only know the regressors approximately and the noise variance is not zero) and that the gradient descent on the log-likelihood loss achieves the same objective. Hence we use the negative log-likelihood function to learn the classifiers, \ie
\begin{align}
&L_{\log}(\bW,\bA) \nonumber \\
&\define  - \Expect_{(x,y)}[\log P_{y|\bx}] \label{eq:logloss} \\
&=-\Expect \log \pth{\sum_{i \in [k]} \frac{e^{\inner{\bw_i}{\bx}}}{\sum_{j \in [k]}e^{\inner{\bw_j}{\bx}}} \cdot \calN(y|g(\inner{\ba_i}{\bx}),\sigma^2)}, \nonumber
\end{align}
where $\bW^\top=\begin{bmatrix}
\bw_1| \bw_2 | \ldots| \bw_{k-1}
\end{bmatrix}$.
Note that the objective \prettyref{eq:logloss} in not convex in the gating parameters $W$ whenever $\sigma \neq 0$. We omit the input distribution $P_x$ from the above negative log-likelihood since it does not depend on any of the parameters. We now define the domain of the gating parameters $\Omega$ as
\begin{align*}
\bW \in \Omega \define \{\bW \in \reals^{(k-1)\times d}: \| w_i \|_2 \leq R, \forall i \in [k-1] \},
\end{align*}
for some fixed $R>0$. Without loss of generality, we assume that $\bw_k=0$. Since we know the regressors approximately from the previous stage, \ie $\bA \approx \bA^\ast$, we run gradient descent only for the classifier parameters keeping the regressors fixed, \ie
\begin{align*}
\bW_{t+1} =\Pi_{\Omega}( \bW_t - \alpha \nabla_{\bW}  L_{\log}(\bW_t,\bA)),
\end{align*}
where $\alpha>0$ is a suitably chosen learning-rate, $\Pi_{\Omega}(\bW)$ denotes the projection operator which maps each row of its input matrix onto the ball of radius $R$, and $t>0$ denotes the iteration step. In a more succinct way, we write
\begin{align*}
\bW_{t+1} &= G(\bW_t,\bA),\\
G(\bW,\bA) &\define \Pi_{\Omega}( \bW - \alpha \nabla_{\bW}  L_{\log}(\bW,\bA)).
\end{align*}
Note that $G(W,A)$ denotes the projected gradient descent operator on $W$ for fixed $A$. In the finite sample regime, we define our loss $L_{\log}^{(n)}(\bW,\bA)$ as the finite sample counterpart of \prettyref{eq:logloss} by taking empirical expectations.
%\begin{align*}
% \define  - \sum_{i \in [n]} \frac{\log P_{y_i|\bx_i}}{n}.
%\end{align*}
Accordingly, we define the gradient operator $G_n(\bW,\bA)$ as
\begin{align*}
G_n(\bW,\bA) \define \Pi_{\Omega}( \bW - \alpha \nabla_{\bW}  L_{\log}^{(n)}(\bW,\bA)).
\end{align*}
In this paper, we analyze a sample-splitting version of the gradient descent, where given the number of samples $n$ and the iterations $T$, we first split the data into $T$ subsets of size $\lfloor n/T \rfloor$, and perform iterations on fresh batch of samples, \ie $\bW_{t+1}=G_{n/T}(\bW_t,\bA)$. We use the norm $\norm{W-W^\ast}= \max_{i \in [k-1]}\norm{w_i-w_i^\ast}_2$ for our theoretical results. The following theorem establishes the almost geometric convergence of the population-gradient iterates under some high SNR conditions. The following results are stated for $R=1$ for simplicity and also hold for any general $R>0$.
\begin{theorem}[GD convergence for classifiers]
\label{thm:twopopW}
Assume that $\max_{i \in [k]} \norm{a_i-a_i^\ast}_2 = \sigma^2 \varepsilon_{\mathrm{reg}} $. Then there exists two positive constants $\alpha_0$ and $\sigma_0$ such that for any step size $0<\alpha \leq \alpha_0$ and noise variance $\sigma^2<\sigma_0^2$, the population gradient descent iterates $\{\bW\}_{t \geq 0}$ converge almost geometrically to the true parameter $\bW^\ast$ for any randomly initialized $W_0 \in \Omega$, \ie
\begin{align*}
\norm{\bW_t-\bW^\ast} \leq \pth{\rho_\sigma}^t \norm{\bW_0 -\bW^\ast}+ \kappa \varepsilon_{\mathrm{reg}}\sum_{\tau=0}^{t-1}(\rho_\sigma)^\tau,
\end{align*}
where $(\rho_\sigma,\kappa) \in (0,1)\times (0,\infty)$ are dimension-independent constants depending on $g,k$ and $\sigma$ such that $\rho_\sigma=o_{\sigma}(1)$ and $\kappa = O_{k,\sigma}(1)$. 
%\leq  (k-1)\frac{\sqrt{6(2+\sigma^2)}}{2}$ for $g=$linear, sigmoid and ReLU.
\end{theorem}
%\begin{remark}\normalfont
%Notice that the above conclusions formalize our earlier intuition that smaller the estimator error for the regressors, the better the estimation accuracy of the classifiers with respect to the true parameters. Moreover, it is quite interesting that with regressors kept fixed at $\bA \approx \bA^\ast$, the classifiers converge to the true parameters with any random initialization in $\Omega$. We did not try to optimize the explicit rate of convergence $\rho_\sigma$ and we believe it might be possible to obtain a tight characterization of this convergence.
%\end{remark}
\begin{proof}(Sketch)
For simplicity, let $\varepsilon_\mathrm{reg}=0$. Then we can show that $G(\bW^\ast,\bA^\ast)=\bW^\ast$ since $\nabla_{\bW}L_{\mathrm{\log}}(\bW=\bW^\ast,\bA^\ast)=0$. Then we capitalize on the fact that $G(\cdot,\bA^\ast)$ is strongly convex with minimizer at $\bW=\bW^\ast$ to show the geometric convergence rate. The more general case of $\varepsilon_\mathrm{reg}>0$ is handled through perturbation analysis. 
\end{proof}
We conclude our theoretical discussion on MoE by providing the following finite sample complexity guarantees for learning the classifiers using the gradient descent in the following theorem, which can be viewed as a finite sample version of \prettyref{thm:twopopW}.

\begin{theorem}[Finite sample complexity and convergence rates for GD]
\label{thm:twosampW}
In addition to the assumptions of \prettyref{thm:twopopW}, assume that the sample size $n$ is lower bounded as $n \geq c_1 T d \log(\frac T \delta)$. Then the sample-gradient iterates $\{ \bW^t \}_{t=1}^T$ based on $n/T$ samples per iteration satisfy the bound
\begin{align*}
\norm{\bW^t-\bW^\ast} &\leq (\rho_\sigma)^t \norm{\bW_0-\bW^\ast}\\
&\hspace{1em}+\frac{1}{1-\rho_\sigma}\pth{\kappa \varepsilon_{\mathrm{reg}}  + c_2 \sqrt{\frac{d T \log(T k/\delta)}{n}}}
\end{align*}
with probability at least $1-\delta$.
\end{theorem}

%
%Notice that above results are in a slightly different vein compared to our earlier results in \prettyref{sec:gradregressor} where we directly analyzed the landscape of $L(\cdot)$. This is because the analysis of log-likelihood surface for latent variable models is technically far more challenging and many of the basic problems for far simpler models such as Gaussian mixtures, mixtures of linear regressions, etc. still remain open. To the best of our knowledge, the only known results in this topic are recent works of \cite{Daskalakis17,hsulengthy}, where they analyzed the log-likelihood landscape for mixtures of two symmetric Gaussians assuming that the mixing probability $0.5$ is known. Extending these results to settings where the mixing probabilities are not known and allowing for more number of mixture component, and generalizing them to mixtures of regressions and finally, MoE problems is an independent and interesting topic of future research.
